New stellar velocity substructures from Gaia DR3 proper motions

Local stellar motions are expected, and have been shown, to include signatures of the Galaxy's past dynamical evolution. These are typically divided into the disc, which shows the dynamical effects of spiral arms and the bar, and the stellar halo, with structures thought to be debris from past mergers. We use Gaia Data Release 3 to select large samples of these populations without limiting them to sources with radial velocities. We apply a penalised maximum likelihood method to these samples to determine the full 3D velocity distribution in Cartesian $(U, V, W)$ or spherical $(v_r, v_\phi, v_\theta)$ coordinates. We find that the disc population is dominated by four moving groups and also detect a new moving group at $(U, V) = (-10, -15)$ km s$^{-1}$ which we call MMH-0. For the stellar halo, we isolate the accreted component with cuts in transverse velocity and the colour-magnitude diagram. In this component we find several known structures believed to be caused by past mergers, particularly one around $(v_r, v_\phi, v_\theta) = (-150, -300, -100)$ km s$^{-1}$ appears more prominent than previously claimed. Furthermore we also identify two new structures near $(v_r, v_\phi, v_\theta) = (225, 25, 325)$ km s$^{-1}$ and $(0, 150, -125)$ km s$^{-1}$ which we refer to as MMH-1 and MMH-2 respectively. These results give new insights into local stellar motions and shows the potential of using samples that are not limited to stars with measured line-of-sight velocities, which is key to providing large samples of stars, necessary for future studies.

==> sections/discussion.tex <==
\subsection{The bifurcated WD CMD}
In Section \ref{sec:intro} we reviewed the literature on the nature of the bifurcation of the CMD in the \textit{Gaia} data. We know that there exists a bimodality in the mass distribution of spectral class DA WDs \citep{kilic18, jimenez19, kilic2020} at around $\sim$0.6 M$_\odot$ and $\sim$0.8 M$_\odot$.

Cooling tracks for these masses of DA WDs would produce a bifurcation that appears very similar to the one visible in \textit{Gaia} \citep{el-badry18}. However, massive WDs will form sooner and begin cooling at an earlier time than the less massive ones, which means that for these cooling tracks to be simultaneously visible in the CMD the massive WDs \textbf{must be a) formed through the merger of lower mass WD binaries, b) cooling slower due to crystallization, or c) formed at a later time.} Scenario a) was suggested by \cite{kilic18} but subsequently dismissed by \cite{kilic2020} due to merger models being unable to produce a mass distribution that fit the observations as well as, perhaps more importantly, not being able to find a significant amount young and massive DA WDs with high velocities. This leaves \textbf{scenarios b) and c). In the first of these scenarios the process of crystallization \citep{tremblay19} will result in a slowdown of the cooling of massive WDs and an observed bimodal WD mass distribution. In the latter scenario a multimodal age distribution could produce massive WDs at a later time for a bimodal mass distribution.} In this case massive WDs would have a smaller velocity dispersion as they have not had as much time to be heated. In our Fig. \ref{fig:mov_disp} it is clear that this behaviour is observed. The velocity distributions for the red and blue sequences in Figures \ref{fig:UV}, \ref{fig:UW}, and \ref{fig:VW} exhibit this as well with the red sequence showing a larger velocity dispersion.

\textbf{Atmospheric composition can elegantly explain the visible bifurcation in the \textit{Gaia} data with an upper DA branch and a lower branch of He-dominated WDs with trace amounts of H or other metals. The bimodal WD mass distribution fits well with this explanation when described by the process of crystallisation. This, however, does not provide the difference in kinematics between the two sequences that we identify.} This difference arises naturally however, \textbf{with} a bimodal WD mass distribution from \textbf{a multimodal age distribution. A detailed study of the age distribution of the WD population would provide valuable insight into this and analytical modelling of WD formation and evolution following bursts of star formation  would be a good avenue to test this explanation.}
\subsection{The velocity structure of WDs}\label{subsec:fv_discussion}
 For the first time, we present the velocity distribution of WDs in the Solar neighbourhood in addition to their velocity moments for. We find that the WD velocity distribution in $\pmb{(U, V)}$ shares many features with the velocity distribution of main-sequence stars when comparing our results to recent maps of the kinematic structure of the Solar neighbourhood like those of \cite{katz}, \cite{kushniruk}, or \cite{antoja2012}. When we separate our sample along this bifurcation we can see very similar velocity distributions, with the notable differences being the red sample having a larger velocity dispersion.

The CMD is also split into three equally sized samples based in their absolute magnitude. The mean velocity distribution of all three subsamples is subtracted from each individual subsample which reveals an unexpected over-density for the faintest sample, {\tt C}, in the region $\pmb{(U, V) \approx (7, -19)}$  km s$^{-1}$. The location does not match conclusively to any of the known moving groups and is only identified in \cite{kushniruk} who attributes it to be a part of the \textit{Coma Berenices} moving group along with two other identified groups. If this feature is limited to fainter, older stars it could suggest its origin is dynamical.  In \cite{coma_b} it is shown that the \textit{Coma Berenices} moving group is not vertically phase mixed and is localized to negative $b$ only, and it is suggested to be due to a recent passing by a dwarf galaxy such as \textit{Sagittarius} which fits well with passages suggested in literature (for a summary see the lower panel of Fig 2 of \citealt{ruiz-lara}).

The double-peaked feature identified in $\pmb{W}$ is limited to fainter stars which should be part of an older sample. The feature is symmetrical around the average vertical velocity which suggests that this feature might be in the brighter sample as a single feature around the mode containing younger, less dynamically heated stars.

Beyond smaller scale structure we find that the velocity distribution is very similar to that of main sequence stars which can be expected since WDs are subjected to the same dynamical processes as other stars. The distributions also show very clear arches like those seen in dynamical studies of main sequence stars (e.g., \citealt{trick1}). To further narrow down the origin of the observed features requires comparison with model predictions or investigating the ages and abundances of their associated stars. For example, It would be possible to investigate the age evolution of dynamical features in the distributions by studying their appearance for several absolute magnitude bins and associating the absolute magnitude with ages using WD cooling tracks.

